Z-ICL: Zero-Shot In-Context Learning with Pseudo-Demonstrations

Although large language models can be prompted for both zero- and few-shot learning, performance drops significantly when no demonstrations are available. In this paper, we introduce Z-ICL, a new zero-shot method that closes the gap by constructing pseudo-demonstrations for a given test input using a raw text corpus. Concretely, pseudo-demonstrations are constructed by (1) finding the nearest neighbors to the test input from the corpus and pairing them with random task labels, and (2) applying a set of techniques to reduce the amount of direct copying the model does from the resulting demonstrations. Evaluation on nine classification datasets shows that Z-ICL outperforms previous zero-shot methods by a significant margin, and is on par with in-context learning with labeled training data in the few-shot setting. Overall, Z-ICL provides a significantly higher estimate of the zero-shot performance levels of a model, and supports future efforts to develop better pseudo-demonstrations that further improve zero-shot results.

==> sections/01-old-intro.tex <==
\begin{figure}
\centering \footnotesize
    \resizebox{\columnwidth}{!}{\includegraphics[scale=0.2]{images/Retrieval Figure_new.png}}
    % \vspace{12em}
\caption{
    An illustration of {\ours} with \SL, %-Nearest with $k=3$,
    %where the LM makes
    making a prediction between \mypos\ and \myneg.
    \ours\ first identifies $k$ nearest neighbors to the test input from a text corpus, % (Section~\ref{subsec:method-retrieval}),
    pairs each sentence with a synonym of a randomly chosen label, i.e., \texttt{good} and \texttt{bad}, %(Section~\ref{subsec:method-labeling}),
    and uses in-context learning. % (Section~\ref{subsec:method-icl}).
    %This is the most basic version of \ours\ (called `\topk'); refer to Section~\ref{subsec:method-retrieval} for other variants. 
    \iz{nice figure. I suggest to change one of the ``good'' to ``bad'' so it doesn't look like you are using the flipped label. Is there enough space in the figure to write ``random labels''? 
    Also, maybe change one or two of the nearest neighbors to be something about customer service but not a customer service review, things like ``Customer service satisfaction report'' or ``Please call our customer support during business hours''  }
    \sewon{+1 on everything what Iz said. Also, maybe we can make better use of the space and make the font slightly larger, e.g., I think the concat icon is too big and can be smaller, and remove some black lines inside the text corpus (not the border).}
}\label{fig:teaser}
\end{figure}

Large language models (LMs) trained on a vast amount of text have shown to be able to perform a new task with no gradient updates, by conditioning on input-label pairs from the training data, so-called {\em demonstrations}~\citep{brown2020language}.
This method, called in-context learning (ICL), is significantly better than zero-shot methods that do not use demonstrations.

Prior work suggests that in-context learning may be mainly about better locating the ability it has already learned during pre-training~\citep{reynolds2021prompt,xie2022explanation,razeghi2022impact,min2022rethinking}, i.e., the demonstrations provide the correct space of the inputs and the labels to better locate the intrinsic, relevant task ability %\iz{``to better locate the relevant task abilities'' (probably remove the word ``zero-shot'')}
of the LM. \iz{This is a fundamental idea in this project. It is worth elaborating here further what we mean by locating abilities }
%
%\citet{reynolds2021prompt} claims that in-context learning is about better locating an inherent capability of the LM, and current zero-shot performance (with no demonstrations) is significantly underestimated.
This implies that current zero-shot performance (with no \demos) may significantly be underestimated, and can be as good as in-context learning.


In this paper, we propose \textbf{\ours}: \textbf{Z}ero-shot \textbf{\textsc{i}}n-\textbf{\textsc{c}}ontext \textbf{\textsc{l}}earning, a new method for zero-shot LM prompting (Section~\ref{fig:teaser}).
The key idea of \ours\ is to construct the \pdemos\ %\iz{can we say ``fake demonstrations'' or ``demonstration-like''?}
%without any
\iz{``labeled''} \sewon{I used ``raw corpus'' because I want to distinguish from ``unlabeled training data'} using a raw text corpus, and use in-context learning.
%\iz{The key ideas of OURS is to use in-context learning with ``demonstration-like'' inputs without any ``labeled'' training data.}
\iz{(We need a name for the fake demonstrations. It will make it easier to refer to. I know you used synthetic-demonstrations before, so we need a term like this but with a different word other than syntehtic.)}
In particular, \ours\ retrieves a set of nearest neighbor from the corpus and assigns a random label to each, which is presumably sufficient to provide signals about the correct space of the inputs and the labels, as the demonstrations from the $k$-shot training data do~\citep{xie2020unsupervised,min2022rethinking}. %\shane{Do we wanna highlight that its still sigificantly better than no-demonstrations? I guess the key question here is how much light we wanna shed on this simplest version. My opinion is to do a little more than now. So instead sort of criticizing this simplest version, we form the story as that the simplest version is already pretty good, but we found managing to reduce the copying effect would further increase our results all the way till close to ICL, especially since we've already decided to include it as part of the method rather than a baseline now.} \sewon{Good point, I added it in the beginning of the next paragraph. How does it look like?}

We find that this simple version is significantly better than a previous zero-shot method with no demonstrations.
%\iz{phrase this in a positive way. Our method achives very good results compared to zero-shot period. Then, mention that we can make it even better by following the copy-effect intuition. Same applies to abstract}
Nonetheless, it lags behind few-shot in-context learning.
%Nonetheless, it is still significantly worse than few-shot in-context learning.
Our analysis reveals that this is due to an observed behavior which we call {\em the copying effect}: when the demonstrations include sentences that are very close to the test input, the LM predictions are heavily influenced by the labels paired with such sentences.
Thus, if the paired labels in the demonstrations are incorrect, the model prediction is also likely to be incorrect.
%This happens regardless of whether the training examples or retrieved sentences are used.
%Section~\ref{subsec:copying-effect} shows a set of empirical evidence that supports the copying effect hypothesis.

To improve zero-shot performance, we carefully design components of \ours\ that prevent the copying effect. 
%
Specifically, we propose two key techniques.
%
The first is to take {\em \pns} (neighbors in the text corpus) of the nearest sentences instead of the nearest sentences themselves, so that the sentences in the demonstrations are from the similar distribution as the text input but are sufficiently distant.
%
The second is to use {\em synonyms} of the labels in the demonstrations, instead of the labels that are used for the prediction at test time, e.g., \{\mypos, \myneg\}$\leftrightarrow$\{\texttt{good}, \texttt{bad}\}. In this way, the model prediction is less affected by directly copying a label from the demonstrations.

We evaluate \ours\ on nine text classification datasets.
Three of them are in the domains that are not coverd by the retrieval corpus, which we set up on purpose to evaluate the generalizability of \ours.
We experiment with GPT-J~\citep{wang2021gpt}, GPT-NeoX~\citep{black2022gpt} and GPT-3~\citep{brown2020language}, whose sizes range from 6B, 20B to 175B.
In a template-free setup, \ours\ significantly outperforms a previous zero-shot method (no-\demos), and \ours+\PN+\SL\ significantly outperforms both of them, consistently across different datasets and LMs.
\ours+\PN+\SL\ is also on par with in-context learning that uses the $k$-shot training data. % with GPT-NeoX.
\shane{"We further conduct ablations showing that"}Ablations show that 
(1) constructing the format of the demonstrations is key to performance: simply conditioning on the in-distribution text works poorly,
(2) our two techniques---\pns and synonym labeling---are critical, since not using either of them significantly hurts performance,
and
(3) performance improves as the size and the coverage of the corpus increase.

Together, \ours\ provides a significantly higher estimate of the model's ability to perform a new task zero-shot, and poses a set of new questions about the capacities of LMs. Our code is available at \url{github.com/Alrope123/z-icl}. \shane{I like the conclusion here more than the one in the abstract}


==> sections/05-table_discard.tex <==
\newcommand{\rt}[2]{$#1_{#2}$}

\newcommand{\rgamzp}{\rt{50.0}{0.0}}

\newcommand{\cjndamzp}{\rt{58.6}{0.0}}
\newcommand{\cjgamzp}{\rt{90.3}{0.7}}
\newcommand{\cjramzp}{\rt{88.9}{1.1}}
\newcommand{\cjrsamzp}{\rt{73.5}{3.8}}
\newcommand{\cjnoamzp}{\rt{76.8}{0.9}}
\newcommand{\cjnamzp}{\rt{86.3}{0.4}}
\newcommand{\cjdnamzp}{\rt{\mathbf{86.9}}{\mathbf{0.7}}}
\newcommand{\cjpnamzp}{\rt{86.4}{0.9}}
\newcommand{\cjdramzp}{\rt{85.5}{0.7}}

\newcommand{\cnndamzp}{\rt{63.2}{0.0}}
\newcommand{\cngamzp}{\rt{90.3}{0.8}}
\newcommand{\cnramzp}{\rt{88.5}{1.5}}
\newcommand{\cnrsamzp}{\rt{70.4}{2.3}}
\newcommand{\cnnoamzp}{\rt{78.8}{0.9}}
\newcommand{\cnnamzp}{\rt{84.0}{0.3}}
\newcommand{\cndnamzp}{\rt{\mathbf{84.5}}{\mathbf{0.9}}}
\newcommand{\cnpnamzp}{\rt{84.3}{0.7}}
\newcommand{\cndramzp}{\rt{82.0}{0.4}}

\newcommand{\dnndamzp}{\rt{50.8}{0.0}}
\newcommand{\dngamzp}{\rt{95.6}{0.5}}
\newcommand{\dnramzp}{\rt{92.9}{2.5}}
\newcommand{\dnrsamzp}{\rt{83.5}{12.9}}
\newcommand{\dnnoamzp}{\rt{87.5}{0.7}}
\newcommand{\dnnamzp}{\rt{\mathbf{94.9}}{\mathbf{0.4}}}
\newcommand{\dndnamzp}{\rt{94.8}{0.3}}
\newcommand{\dnpnamzp}{\rt{94.0}{0.1}}
\newcommand{\dndramzp}{\rt{94.1}{0.5}}


\newcommand{\rgcr}{\rt{50.0}{0.0}}

\newcommand{\cjndcr}{\rt{67.0}{0.0}}
\newcommand{\cjgcr}{\rt{84.9}{2.0}}
\newcommand{\cjrcr}{\rt{81.8}{1.4}}
\newcommand{\cjrscr}{\rt{71.5}{2.4}}
\newcommand{\cjnocr}{\rt{64.8}{0.7}}
\newcommand{\cjncr}{\rt{75.6}{0.7}}
\newcommand{\cjdncr}{\rt{79.0}{0.7}}
\newcommand{\cjpncr}{\rt{\mathbf{80.9}}{\mathbf{0.3}}}
\newcommand{\cjdrcr}{\rt{\mathbf{81.6}}{\mathbf{0.6}}}

\newcommand{\cnndcr}{\rt{57.2}{0.0}}
\newcommand{\cngcr}{\rt{85.5}{2.3}}
\newcommand{\cnrcr}{\rt{78.1}{3.3}}
\newcommand{\cnrscr}{\rt{68.0}{4.2}}
\newcommand{\cnnocr}{\rt{62.4}{0.2}}
\newcommand{\cnncr}{\rt{72.0}{0.5}}
\newcommand{\cndncr}{\rt{75.9}{0.4}}
\newcommand{\cnpncr}{\rt{\mathbf{79.0}}{\mathbf{0.2}}}
\newcommand{\cndrcr}{\rt{\mathbf{80.9}}{\mathbf{0.9}}}

\newcommand{\dnndcr}{\rt{61.5}{0.0}}
\newcommand{\dngcr}{\rt{78.5}{14.8}}
\newcommand{\dnrcr}{\rt{78.5}{13.6}}
\newcommand{\dnrscr}{\rt{72.5}{13.7}}
\newcommand{\dnnocr}{\rt{76.2}{0.3}}
\newcommand{\dnncr}{\rt{88.6}{0.3}}
\newcommand{\dndncr}{\rt{90.9}{0.3}}
\newcommand{\dnpncr}{\rt{\mathbf{91.4}}{\mathbf{0.3}}}
\newcommand{\dndrcr}{\rt{90.8}{0.3}}


\newcommand{\rgmr}{\rt{50.0}{0.0}}

\newcommand{\cjndmr}{\rt{59.2}{0.0}}
\newcommand{\cjgmr}{\rt{85.0}{0.5}}
\newcommand{\cjrmr}{\rt{84.4}{0.4}}
\newcommand{\cjrsmr}{\rt{68.5}{2.9}}
\newcommand{\cjnomr}{\rt{68.3}{0.9}}
\newcommand{\cjnmr}{\rt{77.7}{0.3}}
\newcommand{\cjdnmr}{\rt{77.0}{0.5}}
\newcommand{\cjpnmr}{\rt{\mathbf{77.2}}{\mathbf{0.2}}}
\newcommand{\cjdrmr}{\rt{71.6}{0.6}}

\newcommand{\cnndmr}{\rt{58.7}{0.0}}
\newcommand{\cngmr}{\rt{86.2}{0.8}}
\newcommand{\cnrmr}{\rt{86.3}{0.9}}
\newcommand{\cnrsmr}{\rt{65.0}{4.9}}
\newcommand{\cnnomr}{\rt{63.5}{0.8}}
\newcommand{\cnnmr}{\rt{69.9}{0.5}}
\newcommand{\cndnmr}{\rt{71.9}{0.8}}
\newcommand{\cnpnmr}{\rt{\mathbf{73.2}}{\mathbf{0.3}}}
\newcommand{\cndrmr}{\rt{69.3}{0.4}}

\newcommand{\dnndmr}{\rt{49.9}{0.0}}
\newcommand{\dngmr}{\rt{89.0}{0.9}}
\newcommand{\dnrmr}{\rt{81.2}{13.7}}
\newcommand{\dnrsmr}{\rt{74.9}{8.7}}
\newcommand{\dnnomr}{\rt{71.7}{1.1}}
\newcommand{\dnnmr}{\rt{82.2}{0.4}}
\newcommand{\dndnmr}{\rt{\mathbf{84.2}}{\mathbf{0.5}}}
\newcommand{\dnpnmr}{\rt{84.0}{0.4}}
\newcommand{\dndrmr}{\rt{81.9}{0.2}}


\newcommand{\rgsstt}{\rt{50.0}{0.0}}

\newcommand{\cjndsstt}{\rt{60.8}{0.0}}
\newcommand{\cjgsstt}{\rt{88.4}{0.8}}
\newcommand{\cjrsstt}{\rt{83.9}{2.2}}
\newcommand{\cjrssstt}{\rt{70.3}{2.9}}
\newcommand{\cjnosstt}{\rt{68.2}{0.4}}
\newcommand{\cjnsstt}{\rt{77.5}{0.6}}
\newcommand{\cjdnsstt}{\rt{\mathbf{78.3}}{\mathbf{0.9}}}
\newcommand{\cjpnsstt}{\rt{76.8}{1.1}}
\newcommand{\cjdrsstt}{\rt{74.5}{0.6}}

\newcommand{\cnndsstt}{\rt{61.9}{0.0}}
\newcommand{\cngsstt}{\rt{89.4}{0.9}}
\newcommand{\cnrsstt}{\rt{88.1}{1.6}}
\newcommand{\cnrssstt}{\rt{66.4}{5.2}}
\newcommand{\cnnosstt}{\rt{62.8}{0.7}}
\newcommand{\cnnsstt}{\rt{71.1}{0.3}}
\newcommand{\cndnsstt}{\rt{72.9}{1.6}}
\newcommand{\cnpnsstt}{\rt{\mathbf{74.3}}{\mathbf{0.2}}}
\newcommand{\cndrsstt}{\rt{72.1}{1.4}}

\newcommand{\dnndsstt}{\rt{49.1}{0.0}}
\newcommand{\dngsstt}{\rt{88.6}{5.1}}
\newcommand{\dnrsstt}{\rt{76.9}{13.8}}
\newcommand{\dnrssstt}{\rt{78.2}{9.4}}
\newcommand{\dnnosstt}{\rt{73.8}{1.0}}
\newcommand{\dnnsstt}{\rt{85.4}{0.3}}
\newcommand{\dndnsstt}{\rt{86.9}{0.5}}
\newcommand{\dnpnsstt}{\rt{\mathbf{87.8}}{\mathbf{0.7}}}
\newcommand{\dndrsstt}{\rt{84.7}{0.3}}


\newcommand{\rgteh}{\rt{38.1}{0.0}}

\newcommand{\cjndteh}{\rt{36.8}{0.0}}
\newcommand{\cjgteh}{\rt{44.3}{1.4}}
\newcommand{\cjrteh}{\rt{42.4}{2.3}}
\newcommand{\cjrsteh}{\rt{37.2}{2.0}}
\newcommand{\cjnoteh}{\rt{38.8}{1.0}}
\newcommand{\cjnteh}{\rt{45.0}{0.4}}
\newcommand{\cjdnteh}{\rt{\mathbf{47.0}}{\mathbf{0.4}}}
\newcommand{\cjpnteh}{\rt{46.4}{0.3}}
\newcommand{\cjdrteh}{\rt{46.2}{1.2}}

\newcommand{\cnndteh}{\rt{28.7}{0.0}}
\newcommand{\cngteh}{\rt{47.9}{1.9}}
\newcommand{\cnrteh}{\rt{44.0}{1.1}}
\newcommand{\cnrsteh}{\rt{34.6}{4.9}}
\newcommand{\cnnoteh}{\rt{38.9}{0.5}}
\newcommand{\cnnteh}{\rt{45.1}{0.6}}
\newcommand{\cndnteh}{\rt{45.1}{0.6}}
\newcommand{\cnpnteh}{\rt{\mathbf{46.7}}{\mathbf{0.6}}}
\newcommand{\cndrteh}{\rt{45.0}{0.8}}

\newcommand{\dnndteh}{\rt{30.8}{0.0}}
\newcommand{\dngteh}{\rt{32.8}{6.5}}
\newcommand{\dnrteh}{\rt{33.1}{3.9}}
\newcommand{\dnrsteh}{\rt{\mathbf{36.4}}{\mathbf{9.5}}}
\newcommand{\dnnoteh}{\rt{40.2}{0.9}}
\newcommand{\dnnteh}{\rt{33.2}{1.0}}
\newcommand{\dndnteh}{\rt{34.4}{0.7}}
\newcommand{\dnpnteh}{\rt{35.2}{0.9}}
\newcommand{\dndrteh}{\rt{33.2}{1.2}}


\newcommand{\rgyelpp}{\rt{50.0}{0.0}}

\newcommand{\cjndyelpp}{\rt{60.2}{0.0}}
\newcommand{\cjgyelpp}{\rt{88.6}{1.0}}
\newcommand{\cjryelpp}{\rt{88.8}{1.4}}
\newcommand{\cjrsyelpp}{\rt{76.4}{6.2}}
\newcommand{\cjnoyelpp}{\rt{80.2}{0.5}}
\newcommand{\cjnyelpp}{\rt{87.5}{0.3}}
\newcommand{\cjdnyelpp}{\rt{88.3}{0.3}}
\newcommand{\cjpnyelpp}{\rt{\mathbf{88.5}}{\mathbf{0.4}}}
\newcommand{\cjdryelpp}{\rt{88.5}{0.7}}

\newcommand{\cnndyelpp}{\rt{57.0}{0.0}}
\newcommand{\cngyelpp}{\rt{86.8}{2.8}}
\newcommand{\cnryelpp}{\rt{88.0}{1.7}}
\newcommand{\cnrsyelpp}{\rt{73.0}{3.1}}
\newcommand{\cnnoyelpp}{\rt{79.1}{0.8}}
\newcommand{\cnnyelpp}{\rt{85.5}{0.2}}
\newcommand{\cndnyelpp}{\rt{\mathbf{87.3}}{\mathbf{0.6}}}
\newcommand{\cnpnyelpp}{\rt{87.0}{0.4}}
\newcommand{\cndryelpp}{\rt{87.2}{0.3}}

\newcommand{\dnndyelpp}{\rt{72.2}{0.0}}
\newcommand{\dngyelpp}{\rt{91.7}{3.6}}
\newcommand{\dnryelpp}{\rt{88.5}{4.3}}
\newcommand{\dnrsyelpp}{\rt{85.0}{8.4}}
\newcommand{\dnnoyelpp}{\rt{89.0}{0.8}}
\newcommand{\dnnyelpp}{\rt{\mathbf{92.8}}{\mathbf{0.4}}}
\newcommand{\dndnyelpp}{\rt{92.7}{0.3}}
\newcommand{\dnpnyelpp}{\rt{92.2}{0.3}}
\newcommand{\dndryelpp}{\rt{92.5}{0.2}}


\newcommand{\rgamaz}{\rt{20.0}{0.0}}

\newcommand{\cjndamaz}{\rt{27.3}{0.0}}
\newcommand{\cjgamaz}{\rt{41.6}{3.0}}
\newcommand{\cjramaz}{\rt{39.8}{2.3}}
\newcommand{\cjrsamaz}{\rt{30.6}{2.5}}
\newcommand{\cjnoamaz}{\rt{36.7}{0.6}}
\newcommand{\cjnamaz}{\rt{\mathbf{41.6}}{\mathbf{0.7}}}
\newcommand{\cjdnamaz}{\rt{40.0}{0.4}}
\newcommand{\cjpnamaz}{\rt{40.5}{0.5}}
\newcommand{\cjdramaz}{\rt{38.4}{0.2}}

\newcommand{\cnndamaz}{\rt{27.5}{0.0}}
\newcommand{\cngamaz}{\rt{41.6}{1.8}}
\newcommand{\cnramaz}{\rt{39.8}{1.4}}
\newcommand{\cnrsamaz}{\rt{27.9}{1.9}}
\newcommand{\cnnoamaz}{\rt{34.7}{1.2}}
\newcommand{\cnnamaz}{\rt{37.3}{0.4}}
\newcommand{\cndnamaz}{\rt{\mathbf{38.5}}{\mathbf{0.4}}}
\newcommand{\cnpnamaz}{\rt{37.8}{0.5}}
\newcommand{\cndramaz}{\rt{36.0}{0.9}}

\newcommand{\dnndamaz}{\rt{20.2}{0.0}}
\newcommand{\dngamaz}{\rt{47.0}{2.7}}
\newcommand{\dnramaz}{\rt{45.6}{1.6}}
\newcommand{\dnrsamaz}{\rt{38.7}{3.6}}
\newcommand{\dnnoamaz}{\rt{41.2}{0.9}}
\newcommand{\dnnamaz}{\rt{\mathbf{41.5}}{\mathbf{0.6}}}
\newcommand{\dndnamaz}{\rt{41.3}{0.6}}
\newcommand{\dnpnamaz}{\rt{41.2}{0.4}}
\newcommand{\dndramaz}{\rt{39.1}{0.3}}


\newcommand{\rgsstf}{\rt{21.5}{0.0}}

\newcommand{\cjndsstf}{\rt{24.2}{0.0}}
\newcommand{\cjgsstf}{\rt{39.6}{0.9}}
\newcommand{\cjrsstf}{\rt{38.0}{0.9}}
\newcommand{\cjrssstf}{\rt{26.5}{2.8}}
\newcommand{\cjnosstf}{\rt{27.5}{0.7}}
\newcommand{\cjnsstf}{\rt{27.5}{0.7}}
\newcommand{\cjdnsstf}{\rt{31.2}{0.4}}
\newcommand{\cjpnsstf}{\rt{\mathbf{32.1}}{\mathbf{0.5}}}
\newcommand{\cjdrsstf}{\rt{28.5}{0.8}}

\newcommand{\cnndsstf}{\rt{23.8}{0.0}}
\newcommand{\cngsstf}{\rt{40.8}{1.1}}
\newcommand{\cnrsstf}{\rt{39.9}{1.2}}
\newcommand{\cnrssstf}{\rt{26.8}{3.6}}
\newcommand{\cnnosstf}{\rt{29.9}{0.8}}
\newcommand{\cnnsstf}{\rt{32.0}{0.2}}
\newcommand{\cndnsstf}{\rt{\mathbf{31.9}}{\mathbf{0.5}}}
\newcommand{\cnpnsstf}{\rt{33.2}{0.3}}
\newcommand{\cndrsstf}{\rt{30.8}{0.6}}

\newcommand{\dnndsstf}{\rt{17.5}{0.0}}
\newcommand{\dngsstf}{\rt{43.0}{3.1}}
\newcommand{\dnrsstf}{\rt{37.5}{3.1}}
\newcommand{\dnrssstf}{\rt{37.5}{6.2}}
\newcommand{\dnnosstf}{\rt{34.0}{0.5}}
\newcommand{\dnnsstf}{\rt{33.0}{0.1}}
\newcommand{\dndnsstf}{\rt{\mathbf{34.3}}{\mathbf{0.8}}}
\newcommand{\dnpnsstf}{\rt{33.3}{0.6}}
\newcommand{\dndrsstf}{\rt{29.7}{0.5}}


\newcommand{\rgyelpf}{\rt{20.0}{0.0}}

\newcommand{\cjndyelpf}{\rt{27.7}{0.0}}
\newcommand{\cjgyelpf}{\rt{43.4}{1.9}}
\newcommand{\cjryelpf}{\rt{43.3}{2.3}}
\newcommand{\cjrsyelpf}{\rt{31.5}{1.9}}
\newcommand{\cjnoyelpf}{\rt{37.5}{0.5}}
\newcommand{\cjnyelpf}{\rt{42.5}{0.6}}
\newcommand{\cjdnyelpf}{\rt{\mathbf{42.5}}{\mathbf{0.6}}}
\newcommand{\cjpnyelpf}{\rt{38.7}{0.5}}
\newcommand{\cjdryelpf}{\rt{41.9}{0.7}}

\newcommand{\cnndyelpf}{\rt{28.6}{0.0}}
\newcommand{\cngyelpf}{\rt{43.5}{0.7}}
\newcommand{\cnryelpf}{\rt{43.5}{1.6}}
\newcommand{\cnrsyelpf}{\rt{29.1}{1.9}}
\newcommand{\cnnoyelpf}{\rt{36.9}{0.8}}
\newcommand{\cnnyelpf}{\rt{39.8}{0.9}}
\newcommand{\cndnyelpf}{\rt{\mathbf{40.4}}{\mathbf{0.5}}}
\newcommand{\cnpnyelpf}{\rt{39.9}{1.0}}
\newcommand{\cndryelpf}{\rt{40.4}{0.7}}

\newcommand{\dnndyelpf}{\rt{21.3}{0.0}}
\newcommand{\dngyelpf}{\rt{40.6}{3.1}}
\newcommand{\dnryelpf}{\rt{41.3}{3.5}}
\newcommand{\dnrsyelpf}{\rt{37.1}{2.6}}
\newcommand{\dnnoyelpf}{\rt{39.1}{0.6}}
\newcommand{\dnnyelpf}{\rt{38.9}{0.4}}
\newcommand{\dndnyelpf}{\rt{\mathbf{39.1}}{\mathbf{0.6}}}
\newcommand{\dnpnyelpf}{\rt{38.6}{0.3}}
\newcommand{\dndryelpf}{\rt{37.7}{0.5}}


\newcommand{\rgiave}{\rt{38.0}{0.0}}

\newcommand{\cjndiave}{\rt{46.3}{0.0}}
\newcommand{\cjgiave}{\rt{65.5}{1.7}}
\newcommand{\cjriave}{\rt{64.2}{1.8}}
\newcommand{\cjrsiave}{\rt{53.5}{3.1}}
\newcommand{\cjnoiave}{\rt{55.8}{0.7}}
\newcommand{\cjniave}{\rt{63.1}{0.5}}
\newcommand{\cjdniave}{\rt{\mathbf{64.0}}{\mathbf{0.5}}}
\newcommand{\cjpniave}{\rt{63.6}{0.5}}
\newcommand{\cjdriave}{\rt{63.7}{0.7}}

\newcommand{\cnndiave}{\rt{43.7}{0.0}}
\newcommand{\cngiave}{\rt{65.9}{1.7}}
\newcommand{\cnriave}{\rt{63.7}{1.8}}
\newcommand{\cnrsiave}{\rt{50.5}{3.1}}
\newcommand{\cnnoiave}{\rt{55.1}{0.7}}
\newcommand{\cnniave}{\rt{60.6}{0.5}}
\newcommand{\cndniave}{\rt{62.0}{0.6}}
\newcommand{\cnpniave}{\rt{\mathbf{62.5}}{\mathbf{0.6}}}
\newcommand{\cndriave}{\rt{61.9}{0.7}}

\newcommand{\dnndiave}{\rt{42.8}{0.0}}
\newcommand{\dngiave}{\rt{64.4}{5.2}}
\newcommand{\dnriave}{\rt{63.3}{4.9}}
\newcommand{\dnrsiave}{\rt{58.9}{8.5}}
\newcommand{\dnnoiave}{\rt{62.2}{0.7}}
\newcommand{\dnniave}{\rt{65.0}{0.5}}
\newcommand{\dndniave}{\rt{\mathbf{65.5}}{\mathbf{0.5}}}
\newcommand{\dnpniave}{\rt{65.4}{0.4}}
\newcommand{\dndriave}{\rt{64.6}{0.5}}



\newcommand{\rgoave}{\rt{40.5}{0.0}}

\newcommand{\cjndoave}{\rt{48.1}{0.0}}
\newcommand{\cjgoave}{\rt{71.0}{0.7}}
\newcommand{\cjroave}{\rt{68.8}{1.2}}
\newcommand{\cjrsoave}{\rt{55.1}{2.9}}
\newcommand{\cjnooave}{\rt{54.7}{0.7}}
\newcommand{\cjnoave}{\rt{60.9}{0.5}}
\newcommand{\cjdnoave}{\rt{\mathbf{62.2}}{\mathbf{0.5}}}
\newcommand{\cjpnoave}{\rt{62.0}{0.6}}
\newcommand{\cjdroave}{\rt{58.2}{0.7}}

\newcommand{\cnndoave}{\rt{48.1}{0.0}}
\newcommand{\cngoave}{\rt{72.1}{0.9}}
\newcommand{\cnroave}{\rt{71.4}{1.2}}
\newcommand{\cnrsoave}{\rt{52.7}{4.6}}
\newcommand{\cnnooave}{\rt{55.1}{0.7}}
\newcommand{\cnnoave}{\rt{57.7}{0.3}}
\newcommand{\cndnoave}{\rt{58.9}{1.0}}
\newcommand{\cnpnoave}{\rt{\mathbf{60.2}}{\mathbf{0.3}}}
\newcommand{\cndroave}{\rt{57.4}{0.8}}

\newcommand{\dnndoave}{\rt{38.8}{0.0}}
\newcommand{\dngoave}{\rt{73.5}{3.0}}
\newcommand{\dnroave}{\rt{65.2}{10.2}}
\newcommand{\dnrsoave}{\rt{63.5}{8.1}}
\newcommand{\dnnooave}{\rt{59.8}{0.9}}
\newcommand{\dnnoave}{\rt{66.9}{0.3}}
\newcommand{\dndnoave}{\rt{\mathbf{68.5}}{\mathbf{0.6}}}
\newcommand{\dnpnoave}{\rt{68.4}{0.6}}
\newcommand{\dndroave}{\rt{65.4}{0.3}}

% GPT-3 results
\newcommand{\ctndamzp}{\rt{77.2}{0.0}}
\newcommand{\ctgamzp}{\rt{86.0}{3.6}}
\newcommand{\ctramzp}{\rt{83.4}{4.8}}
\newcommand{\ctrsamzp}{\rt{80.0}{0.8}}
\newcommand{\ctdnamzp}{\rt{88.5}{0.1}}
\newcommand{\ctpnamzp}{\rt{\mathbf{89.1}}{\mathbf{0.3}}}

\newcommand{\dtndamzp}{\rt{88.2}{0.0}}
\newcommand{\dtgamzp}{\rt{97.0}{0.2}}
\newcommand{\dtramzp}{\rt{95.4}{0.6}}
\newcommand{\dtrsamzp}{\rt{\mathbf{97.3}}{\mathbf{0.1}}}
\newcommand{\dtdnamzp}{\rt{\mathbf{93.1}}{\mathbf{0.7}}}
\newcommand{\dtpnamzp}{\rt{93.0}{0.2}}


\newcommand{\ctndcr}{\rt{76.6}{0.0}}
\newcommand{\ctgcr}{\rt{74.2}{7.4}}
\newcommand{\ctrcr}{\rt{73.9}{3.9}}
\newcommand{\ctrscr}{\rt{75.0}{1.2}}
\newcommand{\ctdncr}{\rt{76.0}{1.4}}
\newcommand{\ctpncr}{\rt{\mathbf{80.8}}{\mathbf{0.6}}}

\newcommand{\dtndcr}{\rt{68.4}{0.0}}
\newcommand{\dtgcr}{\rt{79.5}{9.5}}
\newcommand{\dtrcr}{\rt{81.0}{6.8}}
\newcommand{\dtrscr}{\rt{66.6}{12.4}}
\newcommand{\dtdncr}{\rt{67.4}{0.0}}
\newcommand{\dtpncr}{\rt{\mathbf{71.9}}{\mathbf{0.1}}}


\newcommand{\ctndteh}{\rt{36.2}{0.0}}
\newcommand{\ctgteh}{\rt{43.8}{0.2}}
\newcommand{\ctrteh}{\rt{41.4}{2.0}}
\newcommand{\ctrsteh}{\rt{37.7}{0.0}}
\newcommand{\ctdnteh}{\rt{\mathbf{42.4}}{\mathbf{0.6}}}
\newcommand{\ctpnteh}{\rt{41.4}{0.4}}

\newcommand{\dtndteh}{\rt{37.8}{0.0}}
\newcommand{\dtgteh}{\rt{30.5}{8.0}}
\newcommand{\dtrteh}{\rt{42.2}{39.4}}
\newcommand{\dtrsteh}{\rt{\mathbf{35.1}}{\mathbf{1.2}}}
\newcommand{\dtdnteh}{\rt{26.5}{0.8}}
\newcommand{\dtpnteh}{\rt{\mathbf{28.3}}{\mathbf{0.4}}}


\newcommand{\ctndyelpp}{\rt{88.0}{0.0}}
\newcommand{\ctgyelpp}{\rt{91.7}{0.9}}
\newcommand{\ctryelpp}{\rt{90.4}{1.4}}
\newcommand{\ctrsyelpp}{\rt{78.5}{3.1}}
\newcommand{\ctdnyelpp}{\rt{86.7}{0.3}}
\newcommand{\ctpnyelpp}{\rt{\mathbf{87.6}}{\mathbf{0.0}}}

\newcommand{\dtndyelpp}{\rt{96.4}{0.0}}
\newcommand{\dtgyelpp}{\rt{98.5}{0.1}}
\newcommand{\dtryelpp}{\rt{93.7}{2.1}}
\newcommand{\dtrsyelpp}{\rt{97.7}{0.5}}
\newcommand{\dtdnyelpp}{\rt{97.3}{0.1}}
\newcommand{\dtpnyelpp}{\rt{\mathbf{97.7}}{\mathbf{0.3}}}


\newcommand{\ctndsstt}{\rt{80.8}{0.0}}
\newcommand{\ctgsstt}{\rt{88.1}{1.1}}
\newcommand{\ctrsstt}{\rt{84.8}{1.2}}
\newcommand{\ctrssstt}{\rt{66.9}{2.3}}
\newcommand{\ctdnsstt}{\rt{81.6}{0.8}}
\newcommand{\ctpnsstt}{\rt{\mathbf{82.4}}{\mathbf{74.7}}}

\newcommand{\dtndsstt}{\rt{73.2}{0.0}}
\newcommand{\dtgsstt}{\rt{94.2}{0.2}}
\newcommand{\dtrsstt}{\rt{93.9}{0.5}}
\newcommand{\dtrssstt}{\rt{72.7}{19.1}}
\newcommand{\dtdnsstt}{\rt{76.1}{0.3}}
\newcommand{\dtpnsstt}{\rt{\mathbf{78.1}}{\mathbf{0.1}}}


\newcommand{\rgfave}{\rt{47.6}{0.0}}

\newcommand{\ctndave}{\rt{69.5}{0.0}}
\newcommand{\ctgave}{\rt{73.9}{3.0}}
\newcommand{\ctrave}{\rt{72.3}{3.0}}
\newcommand{\ctrsave}{\rt{67.8}{3.0}}
\newcommand{\ctdnave}{\rt{67.8}{1.3}}
\newcommand{\ctpnave}{\rt{\mathbf{73.4}}{\mathbf{0.6}}}

\newcommand{\dtndave}{\rt{72.7}{0.0}}
\newcommand{\dtgave}{\rt{79.3}{2.5}}
\newcommand{\dtrave}{\rt{77.4}{2.7}}
\newcommand{\dtrsave}{\rt{\mathbf{74.2}}{\mathbf{3.6}}}
\newcommand{\dtdnave}{\rt{71.1}{0.4}}
\newcommand{\dtpnave}{\rt{\mathbf{72.7}}{0.3}}


\definecolor{Gray}{gray}{0.85}
\newcolumntype{a}{>{\columncolor{Gray}}r}

\begin{table*}[ht!]
    \centering \scriptsize
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{ll rrrrrra  rrra }
    \toprule
        \multirow{2}{*}{Method} & \multirow{2}{*}{{\em SL}} & \multicolumn{7}{c}{Covered by $\mathcal{C}$} & \multicolumn{4}{c}{Not covered by $\mathcal{C}$} \\
        \cmidrule(lr){3-9} \cmidrule(lr){10-13}
        && CR & Amz & Amz5 & Yelp & Yelp5 & Tweet & Avg & MR & SST2 & SST5 & Avg \\
    \midrule
        Majority && \rgcr  & \rgamzp & \rgamaz & \rgyelpp & \rgyelpf & \rgteh & \rgiave & \rgmr & \rgsstt & \rgsstf & \rgoave \\
    \midrule
        \multicolumn{12}{l}{\textbf{\em{GPT-J}}} \\
        \multicolumn{12}{l}{\textbf{\em{Channel}}} \\
        No-demos && \cjndcr  & \cjndamzp & \cjndamaz & \cjndyelpp & \cjndyelpf & \cjndteh & \cjndiave & \cjndmr & \cjndsstt & \cjndsstf & \cjndoave \\
        Random inputs         && \cjrscr  & \cjrsamzp & \cjrsamaz & \cjrsyelpp & \cjrsyelpf & \cjrsteh & \cjrsiave & \cjrsmr & \cjrssstt & \cjrssstf & \cjrsoave \\
        %%%% ours starts
        \cmidrule(lr){1-13}
        %%%% ours starts
        \ours: \topk  &  & \cjnocr  & \cjnoamzp & \cjnoamaz & \cjnoyelpp & \cjnoyelpf & \cjnoteh & \cjnoiave & \cjnomr & \cjnosstt & \cjnosstf & \cjnooave \\
        \ours: \topk & \checkmark & \cjncr  & \cjnamzp & \cjnamaz & \cjnyelpp & \cjnyelpf & \cjnteh & \cjniave & \cjnmr & \cjnsstt & \cjnsstf & \cjnoave \\
        \ours: \topsample & \checkmark & \cjdncr  & \cjdnamzp & \cjdnamaz & \cjdnyelpp & \cjdnyelpf & \cjdnteh & \cjdniave & \cjdnmr & \cjdnsstt & \cjdnsstf & \cjdnoave \\
        \ours: \pn & \checkmark & \cjpncr  & \cjpnamzp & \cjpnamaz & \cjpnyelpp & \cjpnyelpf & \cjpnteh & \cjpniave & \cjpnmr & \cjpnsstt & \cjpnsstf & \cjpnoave \\
        % \ours: \domainrandom & \checkmark & \cjdrcr  & \cjdramzp & \cjdramaz & \cjdryelpp & \cjdryelpf & \cjdrteh & \cjdriave & \cjdrmr & \cjdrsstt & \cjdrsstf & \cjdroave \\
        %%%% ours ends
        \cmidrule(lr){1-13}
        %%%% ours ends
        \multicolumn{12}{l}{\textbf{\em{Channel}}} \\
        ICL-gold (Oracle)               && \cjgcr  & \cjgamzp & \cjgamaz & \cjgyelpp & \cjgyelpf & \cjgteh & \cjgiave & \cjgmr & \cjgsstt & \cjgsstf & \cjgoave \\
        ICL-random (Oracle)    && \cjrcr  & \cjramzp & \cjramaz & \cjryelpp & \cjryelpf & \cjrteh & \cjriave & \cjrmr & \cjrsstt & \cjrsstf & \cjroave \\
    \midrule
        \multicolumn{12}{l}{\textbf{\em{GPT-NeoX}}} \\
         \multicolumn{12}{l}{\textbf{\em{Channel}}} \\
        No-demos && \cnndcr  & \cnndamzp & \cnndamaz & \cnndyelpp & \cnndyelpf & \cnndteh & \cnndiave & \cnndmr & \cnndsstt & \cnndsstf & \cnndoave \\
        Random inputs         && \cnrscr  & \cnrsamzp & \cnrsamaz & \cnrsyelpp & \cnrsyelpf & \cnrsteh & \cnrsiave & \cnrsmr & \cnrssstt & \cnrssstf & \cnrsoave \\
        \multicolumn{12}{l}{\textbf{\em{Direct}}} \\
        No-demos && \dnndcr  & \dnndamzp & \dnndamaz & \dnndyelpp & \dnndyelpf & \dnndteh & \dnndiave & \dnndmr & \dnndsstt & \dnndsstf & \dnndoave \\
        Random inputs         && \dnrscr  & \dnrsamzp & \dnrsamaz & \dnrsyelpp & \dnrsyelpf & \dnrsteh & \dnrsiave & \dnrsmr & \dnrssstt & \dnrssstf & \dnrsoave \\
        %%%% ours starts
        \cmidrule(lr){1-13}
        %%%% ours starts
        \ours: \topk  &  & \cnnocr  & \cnnoamzp & \cnnoamaz & \cnnoyelpp & \cnnoyelpf & \cnnoteh & \cnnoiave & \cnnomr & \cnnosstt & \cnnosstf & \cnnooave \\
        \ours: \topk 
        & \checkmark & \cnncr  & \cnnamzp & \cnnamaz & \cnnyelpp & \cnnyelpf & \cnnteh & \cnniave & \cnnmr & \cnnsstt & \cnnsstf & \cnnoave \\
        \ours: \topsample 
        & \checkmark & \cndncr  & \cndnamzp & \cndnamaz & \cndnyelpp & \cndnyelpf & \cndnteh & \cndniave & \cndnmr & \cndnsstt & \cndnsstf & \cndnoave \\
        \ours: \pn 
        & \checkmark & \cnpncr  & \cnpnamzp & \cnpnamaz & \cnpnyelpp & \cnpnyelpf & \cnpnteh & \cnpniave & \cnpnmr & \cnpnsstt & \cnpnsstf & \cnpnoave \\
        % \multirow{2}{*}{\ours: \domainrandom} \\
        % & \checkmark & \cndrcr  & \cndramzp & \cndramaz & \cndryelpp & \cndryelpf & \cndrteh & \cndriave & \cndrmr & \cndrsstt & \cndrsstf & \cndroave \\
        %%%% ours ends
        \cmidrule(lr){1-13}
        %%%% ours ends
        \multicolumn{12}{l}{\textbf{\em{Channel}}} \\
        ICL-gold (Oracle)             & & \cngcr  & \cngamzp & \cngamaz & \cngyelpp & \cngyelpf & \cngteh & \cngiave & \cngmr & \cngsstt & \cngsstf & \cngoave \\
        ICL-random (Oracle)   && \cnrcr  & \cnramzp & \cnramaz & \cnryelpp & \cnryelpf & \cnrteh & \cnriave & \cnrmr & \cnrsstt & \cnrsstf & \cnroave \\
        \multicolumn{12}{l}{\textbf{\em{Direct}}} \\
        ICL-gold (Oracle)              && \dngcr  & \dngamzp & \dngamaz & \dngyelpp & \dngyelpf & \dngteh & \dngiave & \dngmr & \dngsstt & \dngsstf & \dngoave \\
        ICL-random (Oracle)   && \dnrcr  & \dnramzp & \dnramaz & \dnryelpp & \dnryelpf & \dnrteh & \dnriave & \dnrmr & \dnrsstt & \dnrsstf & \dnroave \\
        %%%% ours starts
        %%%% ours starts
        % \multirow{2}{*}{\ours: \domainrandom} \\
        % & \checkmark & \dndrcr  & \dndramzp & \dndramaz & \dndryelpp & \dndryelpf & \dndrteh & \dndriave & \dndrmr & \dndrsstt & \dndrsstf & \dndroave \\
        %%%% ours ends
    \bottomrule
    \end{tabular}\vspace{-.1em}
    \caption{
    Results with GPT-J and GPT-NeoX. {\em SL} indicates whether synonym labeling is used. {\em Oracle} indicates the method has access to the training data, thus is not comparable with the rest of the model.
    Covered/not covered by $\mathcal{C}$ indicates whether or not the domain of the dataset is covered by our text corpus.
    \ours\ is significantly better than previous zero-shot (No-demos) on all datasets, and is on par with ICL-gold on datasets covered by $\mathcal{C}$.
    }\label{tab:main-results}
\end{table*}


\begin{table*}[ht!]
    \centering \scriptsize
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{ll rrrrar
    }
    \toprule
        \multirow{2}{*}{Method} &\multirow{2}{*}{\em SL} & \multicolumn{5}{c}{Covered by $\mathcal{C}$} & Not covered by $\mathcal{C}$ \\
        \cmidrule(lr){3-7} \cmidrule(l){8-8} 
        && CR & Amz & Yelp & Tweet & Avg. & SST-2 \\
    \midrule
        Majority && \rgcr & \rgamzp & \rgyelpp & \rgteh & \rgfave & \rgsstt   \\
    \midrule
        \multicolumn{8}{l}{\textbf{\em{GPT-3}}} \\
        \multicolumn{8}{l}{\textbf{\em{Channel}}} \\
        No-demos  && \ctndcr  & \ctndamzp & \ctndyelpp & \ctndteh& \ctndave & \ctndsstt  \\
        \multicolumn{8}{l}{\textbf{\em{Direct}}} \\
        No-demos  && \dtndcr & \dtndamzp & \dtndyelpp & \dtndteh & \dtndave & \dtndsstt  \\
        \ours: \topsample  & \checkmark & \dtdncr & \dtdnamzp & \dtdnyelpp & \dtdnteh & \dtdnave & \dtdnsstt   \\
        \ours: \topsample & \checkmark & \ctdncr  & \ctdnamzp & \ctdnyelpp & \ctdnteh & \ctdnave & \ctdnsstt  \\
        \ours: \pn  & \checkmark & \ctpncr  & \ctpnamzp & \ctpnyelpp & \ctpnteh & \ctpnave & \ctpnsstt  \\
        \multicolumn{8}{l}{\textbf{\em{Channel}}} \\
        ICL-gold (Oracle)   && \ctgcr  & \ctgamzp & \ctgyelpp & \ctgteh & \ctgave & \ctgsstt  \\
        ICL-random (Oracle)   && \ctrcr  & \ctramzp & \ctryelpp & \ctrteh & \ctrave & \ctrsstt  \\
        \multicolumn{8}{l}{\textbf{\em{Direct}}} \\
        ICL-gold (Oracle)   && \dtgcr  & \dtgamzp & \dtgyelpp & \dtgteh  & \dtgave & \dtgsstt \\
        ICL-random (Oracle)   && \dtrcr  & \dtramzp & \dtryelpp & \dtrteh & \dtrave & \dtrsstt  \\
    \bottomrule
    \end{tabular}\vspace{-.1em}
    \caption{
    Results on GPT-3 on a subset of evaluation datasets.
    %
    %
    {\em SL} indicates whether synonym labeling is used. {\em Oracle} indicates the method has access to the training data, thus is not comparable with the rest of the model.
    Covered/not covered by $\mathcal{C}$ indicates whether or not the domain of the dataset is covered by our text corpus.
    %
    We use a basic template, e.g., \texttt{Review:} for both zero-shot baselines and \ours\ for GPT-3.
    %
    \ours\ is consistently better than previous zero-shot (No-demos) on all datasets even with a template.
    }\label{tab:main-results-gpt3}
\end{table*}

% \begin{table*}[ht!]
%     \centering \scriptsize
%     \setlength{\tabcolsep}{3pt}
%     \begin{tabular}{ll rrrrar
%     }
%     \toprule
%         \multirow{2}{*}{Method} &\multirow{2}{*}{\em SL} & \multicolumn{5}{c}{Covered by $\mathcal{C}$} & Not covered by $\mathcal{C}$ \\
%         \cmidrule(lr){3-7} \cmidrule(l){8-8} 
%         && CR & Amz & Yelp & Tweet & Avg. & SST-2 \\
%     \midrule
%         Majority && \rgcr & \rgamzp & \rgyelpp & \rgteh & \rgfave & \rgsstt   \\
%     \midrule
%         \multicolumn{8}{l}{\textbf{\em{Channel GPT-3}}} \\
%         No-demos  && \ctndcr  & \ctndamzp & \ctndyelpp & \ctndteh& \ctndave & \ctndsstt  \\
%         \ours: \topsample & \checkmark & \ctdncr  & \ctdnamzp & \ctdnyelpp & \ctdnteh & \ctdnave & \ctdnsstt  \\
%         \ours \pn  & \checkmark & \ctpncr  & \ctpnamzp & \ctpnyelpp & \ctpnteh & \ctpnave & \ctpnsstt  \\
%         ICL-gold (Oracle)   && \ctgcr  & \ctgamzp & \ctgyelpp & \ctgteh & \ctgave & \ctgsstt  \\
%         ICL-random (Oracle)   && \ctrcr  & \ctramzp & \ctryelpp & \ctrteh & \ctrave & \ctrsstt  \\
%     \midrule
%         \multicolumn{8}{l}{\textbf{\em{Direct GPT-3}}} \\
%         No-demos  && \dtndcr & \dtndamzp & \dtndyelpp & \dtndteh & \dtndave & \dtndsstt  \\
%         \ours: \topsample  & \checkmark & \dtdncr & \dtdnamzp & \dtdnyelpp & \dtdnteh & \dtdnave & \dtdnsstt   \\
%         \ours \pn   & \checkmark & \dtpncr & \dtpnamzp & \dtpnyelpp & \dtpnteh & \dtpnave & \dtpnsstt  \\
%         ICL-gold (Oracle)   && \dtgcr  & \dtgamzp & \dtgyelpp & \dtgteh  & \dtgave & \dtgsstt \\
%         ICL-random (Oracle)   && \dtrcr  & \dtramzp & \dtryelpp & \dtrteh & \dtrave & \dtrsstt  \\
%     \bottomrule
%     \end{tabular}\vspace{-.1em}
%     \caption{
%     Results on GPT-3 on a subset of evaluation datasets.
%     %
%     %
%     {\em SL} indicates whether synonym labeling is used. {\em Oracle} indicates the method has access to the training data, thus is not comparable with the rest of the model.
%     Covered/not covered by $\mathcal{C}$ indicates whether or not the domain of the dataset is covered by our text corpus.
%     %
%     We use a basic template, e.g., \texttt{Review:} for both zero-shot baselines and \ours\ for GPT-3.
%     %
%     \ours\ is consistently better than previous zero-shot (No-demos) on all datasets even with a template.
%     }\label{tab:main-results-gpt3}
% \end{table*}

==> sections/99-discard.tex <==
\begin{table*}[ht!]
    \centering \footnotesize
    \begin{tabular}{l @{\hspace{2em}} l|rrr|rrr|r}
        \toprule
            \multicolumn{2}{c}{\multirow{2}{*}{Method}} & \multicolumn{3}{c}{GPT-J}  & \multicolumn{3}{c}{GPT-Neox} & GPT-3 \\
                                & & ID & OOD & Total& ID & OOD & Total & Total \\
        \midrule
            \multirow{8}{*}{Direct} 
            & Zero-shot  &  \cjndcr &  &  &  &  &  &  \\
            & Gold Label                &   &  &  &  &  &  &  \\
            & Random Label     &   &  &  &  &  &  &  \\
            & Random Sent          &   &  &  &  &  &  &  \\
        \cmidrule{2-9}
            & \ours\ -\topk    &   &  &  &  &  &  &  \\
            & \ours\ -\topsample   &   &  &  &  &  &  &  \\
            & \ours\ -\pn    &   &  &  &  &  &  &  \\
            & \ours\ -\domainrandom    &   &  &  &  &  &  &  \\
        \midrule
            \multirow{8}{*}{Channel} 
            & Zero-shot  &   &  &  &  &  &  &  \\
            & Gold Label                 &   &  &  &  &  &  &  \\
            & Random Label     &   &  &  &  &  &  &  \\
            & Random Sent          &   &  &  &  &  &  &  \\
        \cmidrule{2-9}
            & \ours\ -\topk    &   &  &  &  &  &  &  \\
            & \ours\ -\topsample    &   &  &  &  &  &  &  \\
            & \ours\ -\pn    &   &  &  &  &  &  &  \\
            & \ours\ -\domainrandom    &   &  &  &  &  &  &  \\
        \bottomrule
    \end{tabular}\vspace{-.1em}
    \caption{
    Main Results. All results are aggregated average in percentage. The bigger number is the accuacy (Macro-F1), and the smaller subscripts are the standard deviation. ID=In-Distribution. OOD=Out-Of-Distribution.
    }\label{tab:main-results-old}
\end{table*}

\paragraph{Evaluation datasets.}
\begin{table}[ht!]
    \centering \footnotesize
    \begin{tabular}{l @{\hspace{2em}} l}
        \toprule
            Dataset & Domain \\
        \midrule
            CR      & movie reviews  \\
            Amazon      & product reviews   \\
            Amazon\_polarity  & product reviews     \\
            Yelp-full   & restaurant reviews     \\
            Yelp-polarity   & restaurant reviews     \\
            Tweet\_eval-sentiment   &  tweets    \\
            Yahoo   & forum answers     \\
            Financial\_phrasebank   & news     \\
            MR   &  movie reviews     \\
            SST-2   & movie reviews     \\
            SST-5   & movie reviews     \\
        \bottomrule
    \end{tabular}\vspace{-.1em}
    \caption{
    List of datasets. \sewon{I think having this table makes it very apparent that our datasets are not very diverse :joy: I would remove it and mention a list of datasets in the main text.}
    }\label{tab:datasets}
\end{table}

\begin{table}[ht!]
    \centering \footnotesize
    \begin{tabular}{l @{\hspace{2em}} l}
        \toprule
            Model & Size \\
        \midrule
            GPT-J       & 6B  \\
            GPT-Neox    & 20B   \\
            GPT-3       & 175B     \\
        \bottomrule
    \end{tabular}\vspace{-.1em}
    \caption{
    List of language models.
    }\label{tab:models}
\end{table}


